Modeling and Predicting the Growth and Death of Membership-based Websites

Driven by outstanding success stories of Internet startups such as Facebook and The Huffington Post, recent studies have thoroughly described their growth. These highly visible online success stories, however, overshadow an untold number of similar ventures that fail. The study of website popularity is ultimately incomplete without general mechanisms that can describe both successes and failures. In this work we present six years of the daily number of users (DAU) of twenty-two membership-based websites - encompassing online social networks, grassroots movements, online forums, and membership-only Internet stores - well balanced between successes and failures. We then propose a combination of reaction-diffusion-decay processes whose resulting equations seem not only to describe well the observed DAU time series but also provide means to roughly predict their evolution. This model allows an approximate automatic DAU-based classification of websites into self-sustainable v.s. unsustainable and whether the startup growth is mostly driven by marketing & media campaigns or word-of-mouth adoptions.

==> figs/forum_catholic_org_pred_lambda1.41197801619206e-05_gamma0.000173451588251787_alpha0.004427497485757 <==
%PDF-1.4
%âãÏÓ\r
1 0 obj
<<
/CreationDate (D:20130814184553)
/ModDate (D:20130814184553)
/Title (R Graphics Output)
/Producer (R 2.15.2)
/Creator (R)
>>
endobj
2 0 obj
<< /Type /Catalog /Pages 3 0 R >>
endobj
7 0 obj
<< /Type /Page /Parent 3 0 R /Contents 8 0 R /Resources 4 0 R >>
endobj
8 0 obj
<<
/Length 31318 /Filter /FlateDecode
>>
stream
xœ¼ÝQdÉq%è÷þõH>LÍuw37³×f°vI`4z$ 
©%…h~ý"_÷èn¶¢¤(³8'H~,ž¶ŒÌ¼Y'víºµ/ù¥}ùÇ/ÿßÿ×ãÿÿãŸþïÿòŸ¾üÅo~¸¾^×õåçÿú›¿ø«Çkúåþð×óåúò÷?´/ùøÿü¡­ÿÁ—ÿ󍯗|™þµÛ—?|ÙC¾Æøòû/¿ùå·¯þÔOÚzû:¯ÿøðgn÷?îÇ?·_üÓ{ÿ³üáÏþÜÿìŸøӟŸ÷ùç?ûèÿÓoÏ'çïþôâ"ó§¿û§þãÿÑŸÉßþ·û¿z|èë_ÿÃþ·û¿'öÕæú´<þ‰¿ý×_=þË_ùí?þðŸ{ÿÃßJ·6¾öyâýûãs~Õ8qùîxo?ûàç÷Çíg¼w|ô?øöÓ§nÝÔî/ëÒîÿ°ùû'‡èöù"ÿ9ŸÿãßÜWÀw|öþìï×üjö¥u_ë_ÿêŸÿá¿ûò_õ/¿~üї_ýîoÿø§ÿúë_ÿ͗ßþ囯þñãñ¥öUûþ'þßýíÿòOÿïýå?týò«?üíïÿáýúK{üÇßýý—¿ý»þ‡ÿÿþù_~,Q¾®[·¯CŸŸãǧϿ^þü´=._üù"ï°óçÞ¿êøéÏüóþxiÖüó'úóx|®ŸþüðÇ?ÿ³觏ïÇ?/I[»_Ñxü°ðýý÷å_þøêû÷q»_ðOñþ]ñþø|ZûY||_ÜïO×Oqù®ø÷gó§¸þ,þøÖúòó‹h¨ÕDžüݗÿçË?ýüs?×Äã{­?*þô¹ÿé[sÌöøãùø^¼?gÆߚ÷ÇßöÇÿ¸8þøžʣÄãÿîÿ`í«ØãË÷øüÛýÁÿ~}ä?ýí|õÿfzŽJÚ¼'ŽUûñ!h"Ý×׬=>K6Ré>*éQª­¥Ú³T{½§È§#òéñµj?þb-ՖRm-Õ6ÉŸ¯^¨-÷[Ê+¾zK¥Ÿҏ¿Q
i-Õ~|²Ÿ5¿ò_±ÇjÍÿTÔ¯íª¤»Þo¡%Riyüi"õo™´ÎJÚVí¹^@&í3Ÿž_¯Âëž_[áuϯ£T[Jµg¯|ÖÌ*é(Ô¶¯W¡¶}í¥Ú£T[Kµg©¶¯Ú·®™Ÿö5<Ÿö¯mTÒ½T[JµµTÛJµ}Վõ»À÷§±QI·¨¤‡ä_w¬¿À
é¹:k×z³›I[Tґ¯í×zÁ…t/Õ¥Úª•´]•´j·Ý
H§[©ö¸îk,z*-š¾Jvc¸¾›µét´|úñ»¡öãwÿRí1ó_±ÇÛúRíYzÝ^ª…ڏßýóï<én•´"j«Ýíіø}쑶^Iûª­_Gâ·Xüî_¨-+VHQI‹WÒ³Tûîi¦?çwO3÷û˜ëîi¦Ó½T{"jk©öŒt×⑾{š¹ŽÉ#}÷4"é¹{šÉ|îžf:-…×=wO3¶ÒëŽ|Ë¿ûkº;÷H÷|oÏï»d…\K¯{–^÷ÝÓÌuDéÈ÷Sýñ»«¤û¬¤ïžfò³æ»§™N[éu¯žf²îq÷4óéÕÓ¼|Ý|ȤWO3Ÿ^w4óéÕӼ߰™k,îžæ5W³*"^=ÍK×/ߝŽëîiæÓ½T{"jk©öº£™Oû¨¤WOó'õñ÷§ÛÝÓ̧{©¶"jk©¶•j{¡vßw4ÓéÕÓ̧G©¶"jÏRíÕÓÌ^%ýîifk»§™O¯;šÙ|¬	©Bzõ4"<Ò«§™O¯žæu¿Ùýþ´Ü=Íäß¡tË¿Û{¤Gþ]î#}÷4s¿I>Ò³¥{¤-ù'¾{šÉ´îžf:ݯ[wO3ÖÒ랥×íù×#ù¾bÌÝÓÌÝ{¤ïžf:-¥ÚZªm¥Ú^øœÛîi¦ÓÍóßk¶{šé´äûŠôÝÓL§­ôº£ðº}÷4"¹ïžf:½îhæÓ*•ô,ÕöüÌà#}÷4"éØ=Ítº—jK©öÌ÷öiË÷×éÈ÷×Úuí¦f>ÞkÕG­ºÖª†5W¼ÐÙ\ñÈ·øÚÕvo3ïù¾—ü{¯×ü›¯/Ìl®xah³]}OmæÞû­xá犏ü;Ï—ü ߊÏüáŠF7W¼0»Ù®QÞ\ñÂôæŠÆ7W\óï†V|æߊ­¸×ªG¥ºìÎì+ÙCœùø=ř»ç¸â÷g>^¸ã¹âž¿Õ»XW¥ºîQÎ||äï4¯¸äo5¯ø¬U·Zõ¨TŸ•Ç9V¼çï7¯¸Ôªk­ºÕª{¥ºíçZóñV«~?֑ßÏuäã«
šlÿ®¸åïþÞ÷^+Õýî"âw+4ûë€ï^h>®µê3ïûÎõR<*Õãnˆ&o½¯øêˆâR«®µêÖÓ·kî1
ÏÇ׳â#}«iÅ[þüŠü-øþM™üàgíµ[­zTª·}o4û©k÷…øÈߙ]qÍß¾[&µ×îµ×•êýn'â½V]ò7ÅW|õIÓ_¸~7Jñ¨Tw§ôº?©øýL{>>jÕµöÚ×ÍÒB|=RˆG¥ºÜÒB¼×ªK­ºÖª[­ºWªë}×´_ÒB|uJwß-¿ÇAóñÕ)M_°ºBóñ¨TŸ{$4_wOW—?õædޏ"âZ«>kÕï¹Ðü§.¼·=šýàm†æãR«¾
)ÄW§´_ÒuS0õÞÆ÷|h>ÞjÕG­ºÔªÏZõu#5ý…óû'ô%w§´ïµêR«®µêV«î…ê}Ÿ…Wˆßϊ$ÿ'~Äï‡Eòq©UŸµêV«•êmwJ"oÌñ^xSúˆÂÛÂG\o×±¹…·…¸×ªGåµ÷Ý)ÍÇ{þi—üã:+®µêVèö^yz¤õ±;¥ùx«U¯tJq©UŸµ×nµê…‡HZ—ÊS$+ÞkÕ+ÒGüî"fÚÈî"æã^«•êzßH-Ä×Ó$…¸ÔªÏZu«UJõ¹;¥ÙoÚ¹;¥ÙVswJóñu#5{cå¿;¥ù¸×ªßÒìk·Ý)ÍV·Ý)ÍÇ¥V]kÕï©ù¸Wޜøî"æã­V}T^»ïNi>>kՏίxTªÇý˜I!Þ·qñQ«®µêw§49<ðˆ{­z^û¸v§4¿o¤æãëy"B\·qq+ÜD~ĽR½íNi>ÞjÕG­ºÔªÏü"Ý+îùG»W<*Õûî"&¯÷G¼çŸ,_q©U×ü©ð+nùcáW¼p¦N£r¨ÎŠ·Âlá#~ϔæã2óCàøýh}>n…ñûáúl\öÓõùøýÈIöµË~ä$¿Ïð÷™áù¸×ªGáq›¡û!û|¼×ªKáq›Gü~ä$·Zu¯TŸûððì×}îgíóñQ«.µê÷#'ùøýÈI>…‡}†ÝÒ쳏xÏ?'½âw§49C¾VÀɗôö#~wJóq—Â{ß7R³Õ}wJóÕG卙ïNi>>kÕ­V=*ÕcwJóñûFj>>
³G¼Ò)}Ä+Ò¥Né#…êr•:¥x¥SúˆW:¥¸:fr•:¥¸Wª·Ý)ÍÇ[­z¥S*­Ô)}Ä+Ri¥GNdïMÌþ´'½8±ïµê£V]kÕ+ÒGÜkÕ£R}ïOLیR§TF©S*£Ô)•Qê"Ê(uJEJÒG¼Ò))ÝH•³H1yYö&Åìp ìUŠ…xe¦T´4S*Zš)}Ä+3¥xe¦TöBÅBüî"fã{¥b!ÞjÕG­ºÔªÏZu«U¯<r"VzäDöjÅB¼2S*V9ˆ|Ågáö½ìõŠ…xTޔzéFªì
‹Ùޅì‹Ù¶ì‹Ù+r–,&ïŒÈÙ²˜Ÿ5‹ùøÝ)M6Üñ'_£¾â•Ãy$J‡óÈÞµ˜muJ":¥º·-â½V}Ôªk­ú}8O²G­{åb:¾w.â­V}ÔªŽ(_ñY«nµêQ©ÞK7Rõì^Ì~Ӟå‹ù¸ÖªÏZõ{ÿbþS•ÏüØç"æÎ#^ñ^¸‰¬gc>®µêV«î•êgc>ÞjÕïsJ³_wÙç"æã…sËW¼°ŒqÅ'—7=ë"G¼êÙǘZu­UŸµê÷ùåùø}€y6~¶2æã=¿||Å¥V]k¯ÝjÕ½RÝö9¥ùø}Œy>~cžk­ú}Œyö§ÍYИýYw64f«û>§4ûÚ}ŸSšßǘçã•cÌÕKǘ«—Ž1×½¨1ýuߛñQ«.µê³òædok,Ä£P}î}…xåóy•Ž1Ÿ{ecöŠ{ÄgáðüGÜk¯½rŒùÜkñ^«^™){scú»®•fJg+͔ξ;¥ùø}Œy>>
oNæÞßXˆÏZu«U¿;¥ÙOÝÞáXˆ÷ZõQ«®…·Fsïq,ĽR}orL_ïRê"γË1Ùòšg™c>>kÕ­°Ùgž}ŽÉÛ:ó,tÌÇ+ǘO-c>µtŒù<Kóq¯UJõ³×1¿;¥ù¸Ôªk­ºÕªßÒìw¶;f«Ûî"æã£pwî+Äg­ú=Sš¼ÿ>­tŒùôÒÓ÷soyÌN<â÷Li>^yú~z鑓¹7=¦¿p{Õc:¾w=¦?ø½ì±—Zu­½v«|æ÷ÂÇlÜöÂÇB¼×ªZu­UŸ…gÀm/|,Ä£R}/|,Ä{a»í……¸Öª[íµWž¾·^zúþoµê£Vý~ä$_ÒBÜjÕ£R}/|,Ä{­ú¨U×Zõû'"|ü~ä$Jõ½ð±ïµêR«^™)}Ä­VÝ+Õ÷ÂÇBü~ä$µêR«~wJ"¿
ÙYø˜G¥úܝÒ|¼vaÛYø˜Wç±Y:œÇöÂÇt|/|,Ä[å3o»SšK­ú}8O²ñbVê"Ú^ø˜íÓÚ^øXˆWfJÍK3¥æ¥™ÒG¼2Sj{ácvüÞöÂÇô×}/|,ÄïNiöƒßq­½v«½öJ§Ô¯Ý)ÍÇ+œøUê"ú^øXˆÏÂ/¾>âQyímϔf«·=SšÂÃ>¾>â³VÝkÕ£R}/|,Äï™Òì®ï™Ò|ü¾'šßœäãQ©¾>¦?ó{ácöoXß³7Ð}/|ÌÞýÄga®ò÷ÂT§ï…éø^øXˆ¯NivÛ÷ÂÇB\kÕ­Výž)õ+M"®{¦4¿o¤f?ø½ð±—ZõÕ)-¼ö{¦4Jõ½ð±ïµê£V}ÝHí×ú{:_ÒB|uJ{[¿Ê¦â«SšŽï……x¯¼v»;¥…êZ{íëFj¿WJÅ×#'éø^øXˆ·ZõQ«¾:¥éÏü^øX¨nµ×•ê{ác!¾:¥éOÝ^øXˆk­ºÕ^ûê"fã±>®}`™Ÿóøê"âëFj¿OµNÅ×#'k±SæGe셏…¸Õª¯Néڍ"ù¶‰½ð±ß[¤â«SÚ}ýF"Š¯Né¸ÖÜT|uJñõÈI!¾:¥ã~<_Òu–zªú^øXˆ÷Zu©U×ZõÕ)]‡¡§¾ç÷ÂÇ}¢w"¾>â­V}uJ‡­¿lRñõo…ø¬U_ÒqïFJÅW§4ßñõÈI!>jÕµV}Öª{­zTªëÝ)-Ä{­úº'Zˆ¯Ni!nµêQ©¾>ÊÝéNÅW§tS›iuÆ^ø(÷ÄR*®µêëFjᵯGN
ŸùÕ)MÇ÷ÂÇB¼×ªK­ºÖª[­úꔦߜ셏…øꔦßU…¸ÔªÏZõÕ)÷#Á©øꔦßÏÇÝ)-Ä׍ÔB|=rRˆk­ú¬U÷ZõÈWï×^øXˆ÷Zu©U_œâ«SZˆ{¥ú^øXˆ·ZõQ«.µê³V}ÝH-Ä×#'éø^ø˜ì­øÝ)Íõ¬Vüî"æãZ«nµê^©>v§4oùnáŠ:¥+^蔮øÌ÷*Wüî"æã«Sš|sÒ¯½ð±ïµê#ß1[ñõÈIò-ñŠßÒ|ÜkÕ£R}/|,Ä{­ºÔªk­ºå;f+îù~]¿öÂÇB¼ÕªZu©UŸµê«Sºvb%&V|ÝHMö.úµ>â«Sšl¼¬øꔊ®:©øê"Ê}êe*¾:¥{ý@*¾:¥…xTªï……øz䤗ZõY«nµêQ©¾>â½V}Ôª¯©…øÝ)ÍǽV=
ÕÛ^øXˆ÷Zu©U×Zõu#µ_œ¤ã{ác!ÞjÕG­ºÔª¯N©Èú™•Š¯NiòÎȊ¯Ni:¾>â«SZˆ¯NiöÝEÛñY«¾:¥ÙwVm/|LÇÇÝ)Mð{ác!.…·…m/|,Ä­ð–¸í…éø^øXˆ·ZõQ«.'ÿe¤í…Ù_…Ú^øXˆG¥ú^øXˆ÷Zu©U_Òä ÔŠ[­ú}#5[}/|̶¼Ú^ø8®õî0_ÒÑ×7_*¾:¥…øê">xËÏU®x´BÜöLéý,w*¾9)ÄW§4Û£n{ác!¾:¥Ù{Û"ƒÐ+¾:¥é¸ßÒä3#+¾:¥…¸äöYqÍ?ð²âV«î•ê{ác!ÞòÛ¬øꔦ¿mbý[þ{~/|,ÄïGN²ì^ø˜÷½ð1ûÁ÷½ð±µêZ«>kÕ½R}/|,Ä[þq›ù‡}V\jÕg­ºÕªG¥z¿;¥ÙŸu}/|,T_œâZ«¾:¥ÉǬV|uJñÕ)Íþœï{ácºú¸;¥…¸T>ó{ác!¾:¥…øꔦ_û^øXˆ·Êkßq)¼-|Äg­ºÞõ½ð1ý™ßñž
{ÅGåµï……ø¬U÷Úg>*Ÿù½ð1ý£r/|,Ä¥V]kÕ­V½ðô}ïgáã½J-¿7:åã÷á<ùø}8O>>kÕ½V=*ÕÏÂÇ|¼×ªK­ºÖªß‡óäã«Sšþ+r/|Lÿ¤ÝÓ×û^øXˆKå
yì™Ò|ÜjգЯ{ácöwر>f{c/|L>û¿â•NéØŸºJ§tuÖ+Ÿù½ð±ÙØq­U·Zu¯Tßñ»Sšýžï»Sš¼71öÂÇBüî"æãVxàe셏éø^øXˆ÷ZõQ«®µê÷#'Ù/Ü^ø˜þ¦ÝÓÕ÷ÂÇôkßq©UŸµêV«•ê{ác!~?r'çYñÂá<+>kÕ½V=*Õç~ú>ïù''W\òÏA¯¸Öª[­ºWªï……x«UµêR«>O"½ð±Jõ½ð±/<}¿â…§ïW¼ðôýŠž¾_q¯¼9ÙÓñ½ð±ïµêR«~wJsç×­øÝ);1‹Ý)MÆåÚç"&'½ð±_ÒB\kÕg­º×ªG¥zÛOßçã½Vý¾'šk᭑셏…¸Wªï……xe¦TöÂÇB\jÕg/ÅÍJñ¨Tß"G­øê"â£V]kÕï§ïs'F®øýô}>~Γýà÷ÂÇB¼×ªK­ºÖª[þ¤Ð¯<}/Zzú^öÂÇB|äÏl\q©UŸµêV«•ê³rNéŠÎ)]ñÂ9¥+®…^d–9'½ð1ßñV«>jÕ甮xáœÒ·ü™+~?r'ï…És‰Wüî"æã£ð "셏…ø¬U÷Úk/œSÚ%J‡óH"ç'(Î#Q:œGöÂÇBüî"&¿pº>f¿mñV8J÷ÂÇì;+ݳ¿Mèõì"fãV«^é"j+uJµ•:¥x¥SúˆW:¥º>â•N©¶R§T{©Sª½Ô)Õ^ê">âZ]xÄ­0º {ác:¾>â½V}Ôªk­ú¬U÷Zõ¨Tßñû'"d{_÷ÂÇB\kÕ­VÝ+Õ÷ÂÇìa›x+œÕùˆWÎ)Õ½ð1;¨{ác¡ºfUK3¥º>fÇïu/|ÌÄê^øXˆk­zå'--|\ñÂÂÇ®¥…+ÞkÕW\Û<âVxØç÷JõÒÂÇ/,|\ñÂÂÇ—ÂÃ>ZZø¸âV«…[ØûéûäºFésÝÓï¨÷ÂÇBÜjÕ½P}…xe¦ô¯Ì">╙Òy=çÉÆ+‡óÌ«t8Ïl¥™ÒÙJ3¥³´ðqÅ+3¥xe¦tž…ùx¦ûæYø˜WfJg/͔νð1ûËÈÜq¯Tûéû|ü~ä$¿9ÉÇ¥ðÀËÜq«U¿Ÿ¾Oþ=e?}Ÿ÷Zõûpžä¯Às/|LêöÂÇBÜkÕ£R}/|,Ä{­ºÔªß‡óäãVè˜M-=r2÷ÂÇB¼×ªZu­UŸµê•Ns–9™Vzädž…É[Zø½ð1y;ož…ùø=Sšœ³šgá£ån¤Nß3¥ÉÛ¸ó,|ÌÇGá&ò<óñY«nµêQ©~>æã½V}Ôªkaºož…ù¸×ªG¡º…ÉÖÎÂÇä;óñ{¦4¹ÌÎÂÇäÁÂv>fãgác>ÞjÕï™Òì§î,|ÌÇï™Òì×½í™Ò|<*Õ÷ÂÇB¼rŒ¹õÒ1æÖK3¥¶>^ûÝ)ÍÆGi¦ô¯Ì"Ú^øXˆKaºÏöÂÇB¼2Sj£4Sjgác>ÞkÕG­ºÖªW>Zmá£Õ>Zmá£Õ>Zmá£Õ>>╙R«-|´ÚÂG«-|´ÚÂG«-|´ÚÂGÛñ¨TßÓoöÂÇìïï¶>âçpžTïÂì9Sš{­zTªûs¦4ïµêçFj6~çÉÆ­V=*Õ÷ÂÇô7í^øXˆÊkÝ)Mÿ["9±½ð±Bußñ^«.µêZ«nµê•NÞJœø^ø˜íø^øXˆWçñö|ú>·Úk¿;¥É¿ß½ïNi>~?r'ßœd_{/=râ½t8ï……xT^û^øXˆ÷Êk»SškၥGN|/|LÇ÷ÂÇì؆…ø¨U—ZõY«~?r'ßœdã{ácúë¾>âR«®µê•™ÒG¼2Sê³4Sê?.|ÌÆÏá<Ù¸Ôªßǘg¿p{ác!•êVš)}Ä+3¥¾>âZyc¶>╙R·ÒL©{i¦Ô½4SúˆKáX¤G\‡2ù^øXˆ{áh ßñV«^yúÞ÷ÂÇB|Öª[­zz•q•Ž1«tŒy\¥Ni셏…ø¬U÷Zõ»Sš<q"öÂÇló!öÂÇB\jÕ+‡óÄ^øXˆG¥ú^ø˜×yÄïNiöëÞw§4¿o¤æ?øY˜-Œ½ðqÜC~©xåpžØñ^«.µêZ«^¹'{ác:¾>╙ҐÒLiHi¦4¤4SúˆWfJñÊLi셏…x/Üƍ½ð±¿;¥ÙŸ6{ácúg–:¥±>¦«ÏÝ);ö½ð±¿çÉÇ+ÒØÕ½pbd셏…x«|æmϔæã•sJc/|,ĽòÆl/|LÇ÷ÂÇB¼2S^zú>¼4SúˆWÎ)½ðQÚº¯–ˆï……x«¼5ŠÒLi셏…~Ö^ûꔮC±"üꔊ¯;[ß×uwJñõÈI!¾:¥…¸ÖªÏZu¯UJõvwJñ^«¾n¤â둓BÜjÕ½R}/|,Ä[­ú¨U—Zõu#µ_œâQ©¾>â½V}Ôªk­ú¬U÷Jõ½ð±_ÒB|Ôª¯N©Üg­¦â…NéŠ:¥+^蔎Kw§4/<r²â…GNV¼ðÈɊÏZu¯U/tJÇ5+Ò/tJW¼Ð)]ñu#5}ÅÍJ§tŝÒqY¥Sºâ­òÚ÷ÂÇB|uJ"¿Œ¬øê"âëFjáƒ_œÈ}"["¾>â…NéŠ:¥+^xú~ÅO߯xáéû/<}?®³ð1wCmÅ{þ6îŠKþ	ô×üè+nùÇmVÜóÛŒ¶>&[^+Þò]â/<r²â÷#'ÉÏ|Ûq¯UÊkßӟù½ð±/tJW¼pNéŠ>®xaáãh¥…+^˜)]ñÂLéŠ>®øýô}nÞfÅï§ï³—ÌYø˜Ÿ…–º·â÷á<¹Û:+^8œgŵ𦴍ÊÓ÷+^xú~ÅOߏv>æã½ð椝…ù¸Öª[­º{úÖÆh{áãÚ´Úrñ»Sšümâ¿;¥ùøº'ZˆßÒ|ÜjÕãߨ¾Þ{<þÇ?û×?ýÝ?=þ[{üæúóýÍ_üÕ¿[ªïÕUÙîZß««
ñ¨Tß««
ñ^«>jÕµV}ÖªWZÂ}¯®JÇ÷êªB¼×ªK­ºÖª[­ºWªûw¾B¼šñ}¯®*ĵV}Öª{­zTªËý;_!ÞkÕWK¸לBß««
q¯Tß««
ñV«>jÕ¥V}æºV†gW¼0<;ú¬Ⱥâ…YW¼ò;_Ÿ¥ßùñÊï|¸çŸ¥[ñÈ?S5º•~çÛG¥Wâ•ßùº•~çëVú¯[åĵѽrâڊ·üøꊏüègW|Öª[­zTªGåĵ/œ¸¶â£p#¢—VW­xᘁ/30FiuՊVW­xauՊVW­ø¬U/¬®ZñÂêª1J««V¼pÌÀŠVW­xauՊVW­¸×ªvSŒQZ]µâ…cV¼°ºjŵVÝjÕ½R}¯®*Ä[­ú½º*w¬ÈŠ‹§—C®ø½º*·Zõ¨T?««òñ^«>jÕµòu—灬¹ï:yȚG¥º>dÍÆ{­ºäÏ<[qÍo²]ñûĵûœ‡T|
Ϧã{uU!ÞkÕG­ºÖªÏZu¯UJõ½ºªÅj¥âkx¶—Zu­U_Òv¡¦â«SšŽïÕUéÞïNi!¾:¥éo›½ºª_ÒBÜjÕ£R}¯®Jnk_ñÕ)-ÄG­ºÖªÏü¢û_óɍå+¾:¥É­žCöêªäá"+¾:¥Ù¿ßåªȺâš?vÅ­VÝ+¯½Ud]ñ–?vÅGám¡œÕUùø¬U·Zõ¨Tï•×V¼2<+½4<+guU²Í+guU>î•ê£Ô)•Qê">â•Né#^é"ÊY]•W:¥2JR'R§T¤Ô)•½º*ýWä^]•m><â«SZˆ¯©…øžMÇ÷êªB|uJ³ïmd¯®*T×Úk_ÒäÞì÷JõywJ³oÈe¯®*ÄïNi>.µê³VÝjÕ£RÝv§4ïµêëFj!®…Ž™ìÕU…¸×ªG¥ú^]Uˆ÷Zu©UŸ…Ž™ìÕU…x¥S*{uUö7hÙ««²]bÙ««
q­UŸµêw§ôâQxk¤{uU¶ºîÕUÙ×®{uUöÛF÷êªB|uJ¼W^{»;¥…øº'ZˆÂ3Ý««Òß6{uU!~wJ³ßó{uUöm¡žÕUÉßeñ^¸þˆvS¬xauՊVW­xá@֏Jõ³º*/¬®ZñJ§ô¯tJu"ŽÐñ<f W]JÇ¨"ŽP)uJUJR•R§ô·Â\å#~wJ"ý:Ý««²Gk¨Vd]q)œ}¥Z9uŲ®¸WªŸÕUùx«U/ȺâR8}J÷êªBÜjÕ£Rý¬®ÊÇ+'®=â•×ñ{¦4{½ÿ¸º*÷ÃêÇÕUÙxTªÿ¸º*ïµêR«®µêV«~?r'ý¶9««òñV«>jÕÅÞÕUÙÏüY]•G¡úüquU6ÞoJçUzädžÕUùø¬U÷Zõ¨ToϙÒl¼5šgu•åNâ™guU>nµêQ©ÞK²Î³º*µêZ«¾n¤fhœ{uUötɹWW¥ã{uU!ÞkÕï§ï³ŸºÒꪷ›ÒGÜ+ÕK««V¼°ºjÅ««Vü>5û…Û««Òß6{uUöáý¹WW¥ãzwJñÊá<³´ºjÅ+²N-È:µt ëÔҁ¬s–ž¾Ä+Oß?╧ïçY]•[á)ìYZ]5æY]•<epžÕUÙ7'guU>.µê³VÝ+oÌÎêªìg¾´ºjÅ+Òé¥Né,­®ZñÕ)Mÿçw§4½›"o•7¥¥ÕU+^é"Î(uJçY]•íQxSjguU>ÞkÕGáœ~;««òñY8§ßÎêª{·H*~¯®ÊÆÏêª|¼²ºê—›ÒG\kÕ+««¬¶ºÊj««¬¶ºÊöêª5ô"y6ÐöêªB|Öªßç"Þ³b©xeu•ÕVWYmu•ÕVWYmu•ÕVWYmuÕ#^9§ÔÎêªì·ÍY]•KáÌFÛ««
Õ­öÚ£R}¯®*Ä{­ú¨U_7RñÕ)ÕûÁT|uJñ»Sšýà÷êªB¼×ªK­ºÖª¯©…øzä$ß««
ñÕ)]wñS?möêªB\jÕg­ºÕªG¥ú^]Uˆ¯Ni!>jÕµV}Öª{­zTªÇÝ)-Ä׍ÔB|=rRˆk­ºÕª{¡ºïÕU…x«U…7¥¸ޔúU:ÆܯÒ1æ~•Ž1÷½º*Ûúð½º*Ûxñ½ºª×Zu»òûX|¯®Ê¶¼ü¬®Jvý¬®²\ƒÝÏê*]o°Rñ»Sšœ9ñ³º*¹<Êk««¼ï™Òäáº>öLi>ÞGyûY]•k­ú¬U¯cîã9SššÞw)SúˆWÎ)u)=râRzäÄ¥t8ïÕUéø^]•=]Ç÷êªìÙ>¾WWâR«>ù^]UøÔEáÄHŸw§4ýÁÏ»Sš}¸ï¿Ÿ¾O>ZøˆßOßçã÷Ó÷ùÞ+_w»o¤â«SšþºÛÝ)-Ä¥V}Öª[­zTªû~ú>_7Rñûpž|\kÕg­º×ªG¥zì§ïóñ^«.µê÷á<ùø}8O>î…êqíÃyòñûéûäÊG|žÄ+Oß?â«Sš=Ó)öÂÇB<
§eÆ^ø˜~í{ác!>jÕµV}Öª{­zTªï……ø}8O>^9œ'öÂÇB¼rŒy셏éø^øXˆ·ZõÊ1æ1JǘÇ^ø˜þ¶Ù³oÈc/|LÇ÷ÂÇô_R{ác!.µêZ«n…7'±>¦ã{ác!ÞjÕG­ºÔªWÎ)}Ä+ç"ÆYø˜ÏÒá<1K‡óÄ,Îgác>>kÕ½V½Ò)
+ÎV:œç¯tJÃJÒ°R§4¬Ô)³ð1oµê£V½r8OxépžðÒ1æá¥cÌ#þÍcÌÿçý7ÿæïXûÚ¿²êÝçú×ÃuÆíÿÿò›ÖÃÇ?ûþ×vÿëoþâ¯ÿӟþ!k~øq·¹nKüáÏùûï§Ã$®	C‹Å£°¨húá"ÑXtƒÄq±Ø`ì,…Eeñ\'ñy‹c(‹
ÆÎâ`Q`Tç+>~â×i,:‹¢^,6;‹ƒEQYœ	¶
Fg1Pœ‹Åã`Q`Tgý-ŒÎbhŒÅã`QXTçÇ9^Ó`tƒD¿`l,vŒÂ¢Â8Y<—¤Àé0‰qÁØXì,…EeqÂh/©Ÿ§Ãî]Þ6;‹FaQYœ0Ú;œ ³(¶‹Åcgq°(0*‹F«ÓÞ¢³(žy3ŒÅÁ¢À¨,N­NMg1P<f6;ŒƒEQYœ,ÚLJÎbxæÍl,v‹Â¢Â8Y4ýåú<ƒÄ3o†`c±³8`ÆÉ¢±è/Ù>À ñ̛!ØXì,…EeqÂh,ú;ì‰gތÀcgqÀ(,*‹FcÑŠgތÀcgq°(0*‹FcÑ?NyÍ@ñ̛ØXì0Feq²h0:šg ç̛}œò0#°±Øa,
ŒÊâdÑ`tÏ%9Ñ<óf6;ŒƒEaQaœ,ŒÎb¼C«ớ!ØXì,…E…q²h,:Œ' 'xæÍl,vŒÂ¢²8a4ƨ3Þá™7#°ÁØY0
‹Êâ"ÑXt£L½^ờØ`ì,FeqÂh,:‹â™7Ógc±Ã8X•ÅÉ¢Áè,Šv½dÿ<‹ÆÁ¢°¨0N
Fg1Hôë%ÇØXì0…E…q²h0:‹Ab\	Ê[l,vŒÂ¢Â8Y4Æ PŸóf%êk6;‹FaQYœ0‹cØ®s¾fƒ±³8`•Å	£±è,ŠýBÓŒÅÁ¢À¨,NEg1P‹í%ýóì0Feq²h0:‹â0#°½Ãø;ŒƒEaQaœ,ŒÎbøœ7°}?ç•a‡q°(,*Œ"EcÑaϼ'­Îö;‹FaQaœ,‹cxæÍlhöÃÎâ€QXT'ŒÆ¢Ã$žy3Œçp…EeqÂh,:‹â™7#°ÁØ_R>ÏÁ¢À¨,NEg10œÏy3‹ý%õ,
ŒÊâdÑ`tÅ3`F`c±¿Ã™á`QXT'‹£³$žy3‹½N{ÍÁ¢°¨0NE‡1H<óf6ûÇé¯9`ÆÉ¢±è0‰gތÀcG3ŒÂ¢²8a4Æ ñ̛Ø`ì,îKÒ®ÏSXT'ŒÆ¢³(žy3ŒÅñ'íó•Å	£±è,ŠgތÀÆb‡q$Ø3•ÅÉ¢Áè,ŠgÀŒÀÆb‡qÔ9Þ¢°¨0N
Fg1H<óf6;Œãã"×ÆÉ¢±è0…öœ7C°±ØY§
‹
ãdÑXtƒÄ3oF`ƒ±³8`<×à"SYœ0‹cxæÍl0v‹ò'ö*‹FcÑYϼ
ÆÎâ`QÞ¡g¨,NEg1P<f6;ŒƒEI0Þ¢²8Y4Å@ñ˜ØXì0¥L¿Þ¢Â8Y4Å ñ̛!ØXì0åãl¯©0NE‡1H<óf6;‹FA³*Œ"EcÑaϼ
ÆÎâ€QXԗŸç"ÑXtƒÄ3oF`ƒ±³8XõÊ8a4ÅÀПóf6;‹ƒEQÔ'‹£³(ž3‹ÆÁ¢À¨uη8Y4Å@ñ˜ØXì0…E­Ó^s²h0:‹Aâ™7C°±Øa,
‹úqúádÑXtƒÄ3o†`c±³8`Æs
œÆ¢Ã$žy3ŒÅ£°¨,ÎWŒë4Æ ñ̛Ø`ì,Feq¾Ã–¡±è,ŠgތÀcgq°(0*‹3Áž¡Áè,ŠgÀŒÀÆb‡q°(0*‹³Îñ
Fg1H<óf6;ŒƒEaQaœ§¼¦Áè,…ñœ7C°±Øa,
‹
ãDSE‡1H<óf6;‹FaQaœ,žkpÂé0‰gތÀcgqÀ(,*‹F{Iû<Æ ñ̛Ø`ì,FeqÂh	z†Îb xæÍl0v‹£²8Y´ã-:‹â0#°±Øa,
ŒÊâdъ¼wr¼¤³$Þóf6;ŒƒEaQaœ,ÚÇٝŠÑ.‹Å£°¨0N
Í~è0‰~ÁØXì,…E…q²h,žKr|žAb\,6;‹FaQYœ0‹þ'òƒ~íy3
ŒÅÁ¢À¨,NE‡úŠíb±ÁØY,
ŒÊâdÑ`ôg†b¿Xl,v‹£²8Y4½N{‹Aâ¸`l,v‹Â¢Â8Y4ýãô×傱±ØY0
‹
ãdÑXô3ƒD½`l,vŒÂ¢²8a4Æ}
¶Í3oF`ƒ±³8`•Å	£±è0Æ;lužy3ŒÅÁ¢À¨,NEg1ÞaOð̛Ø`ì,Feq²h0:‹'àx‡gÀŒÀÆb‡q°(0*‹"EƒÑYŒ:åßg{Λ!ØXì0…E…q²h0:‹ñqêKžy3‹Å£°¨0NE‡1М›gÞÁÆbgqÀ(,*‹FcÑaϼY38ŒÅ£°¨,NEg1P"ë%ýól0v‹£²8a4Å@Q¯w`ƒ±³8X•ÅÉ¢Áè,Šóú~ö+ÃÆb‡q°(0*‹"EƒÑYíJ°½ÅÆb‡q°(,*Œ"EƒÑYýª³¿fc±³8`ÆÉ¢±è0‰q}œã°±ØY0
‹Êâ"ÑXtƒÂþœ7RŒÅ£°¨,NEg1Pl‹ç'Ôϳ³8X•Å	£±è,ŠgތÀö'óóì0Feq²h0:‹â0#°½Cû;ŒƒEQYœ,ŒÎbxæÍl	z†ÆÁ¢°¨0N
Fg1H<óf¶:ã-vŒÂ¢Â8Y4Æ ñ9o`û4ÇõšÅ£°¨,NE‡1H<óf¶³vŒÂ¢²8a4Å@ñ̛Ø`<×`‡s°(0*‹FcÑYϼÅsIŽÏs°(0*‹"EƒÑYÇsÀŒÀÆbIù‹Â¢Â8Y4Å ñ̛!ØXìïP3,
‹
ãdÑ`tƒÄ3o†`c±'830
‹
ãdÑXtƒÄ3o†`c±×ioqÀ(,*‹FcÑaϼ
Æþqúk…EeqÂh,:‹â™7#°ÁØьÃÁ¢À¨,NEg1P<óf6;Œû"NQYœ,ŒÎb xÌl,vÇK¶ÏSXT'‹£³$žy3‹Æñû(,*Œ"EcÑaϼ'ÅÎâxÉñ
‹
ãdÑXtƒByΛ!ØXì,Žw(
‹Êâ"ÑXtƒÄ3oF`ƒ±³8Ô·(,*‹FcÑYϼ
ÆÎâ¨s¾EQYœ0‹Îb xæÍl,vÇÇi¯)0*‹"EƒÑYπÅã@Ó…E…q²h0:‹Aâ™7C°±Øa,žk0àT'‹Æ¢Ã$žy3‹Å£¼¢^Ÿ§Â8Y4Æ ñ̛Ø`ì,å¶PYœ0‹cxæÍl0vŒ'`ÏPYœ0‹Îb xæÍl0v‹'àx‹Êâ"ÑXtC}ΛØXì0¥NyMeq²h0:‹â0#°±Øa,JúÆÉ¢Áè,‰gÞÁÆb‡q°(ç|M…q²h,:ŒAâ™7C°±ØY0
šv¨0NE‡1H<óf6;‹Fañ\'ç"ÑXtƒÄ3oF`ƒ±³8Xõ%ãóœ0‹Îb xæÍl0v‹£¾Áy}€FcÑYπÅã`Q`Ô[†"EƒÑYπÅã`QXÔû[œ,ŒÎbxæÍl,v‹Â¢Ö9^s²h,:ŒAá|Λ!ØXì,…E­S^s²h,:ŒAâ™7#°ÁØY0
‹úqêkNE‡1H<óf6;‹ƒEQќ‡FcÑYϼ
ÆÎâ`Q`TÏ%ipŒÎb xÌl,v‹£²8_Ò?OƒÑYπÅã`QXTç;ŒÐ`tƒÄ3o†`c±Ã8XÆùíúE‡1H<óf6;‹FaQaœ	¶E‡1H<óf6;‹FaQYœ	ö·h,:ŒAâ™7#°ÁØY,
ŒÊâ¬s¼¦±è,†öœ7#°ÁØY,
ŒÊâü8å5
Fg1P<f6;ŒƒEQYœhê¡Áè,‰gÞÁÆb‡q°(,*ŒÍyh0:‹Aâ™7C°±Øa,
‹
ãdñ\'§Ã$žy3‹Å£°¨0Ní%ýótƒÄ3oF`ƒ±³8`•Å	£½ÃøÆ ñ̛Ø`ì,FeqÂhßO¿2tÅ3oF`ƒ±³8X•ÅÉ¢½Ã–¡³(ž3‹ÆÁ¢À¨,N-ÁþÅ ñ̛!ØXì0…E…q²huŽ×tƒBΛ!ØXì,…E…q²h§¼¦Ã$žy3‹Å£°¨0N
M=tƒÄ3oF`ƒ±³8`•Å	£¡9Æ ñ̛Ø`ì,FeqÂh,žKÒàϼ
ÆÎâ`Q`T'‹£¿¤žâ0#°±Øa,
ŒÊâdÑ`ôw`xæÍl,v‹Â¢Â8Y4ýûW†Aâ™7C°±ØY0
‹
ãdÑXôwØ2ϼ'ÅÎâ€QXT'ŒÆ¢'ØßbxæÍl0vŒÂ¢²8a4½ÎñšAa<çÍl0v‹£²8a4ýã"×ϼ
ÆÎâ`Q`T'‹£œúšâ0#°±Øa,
ŒÊâdÑ`t4çaxæÍl,v‹Â¢Â8Y4Ås
šgÞÁÆbgqÀ(,*Œ"EcÑaŒ—ôớ!ØXì,…EeqÂh,:Œñ'ñqžy3ŒÅ£°¨,NEg1þ5ïÃ'çÍ(l0v‹£²8a4Åx‡-A¿Xl0v‹£²8Y4Åx‡=Á¸Xl,v‹£²8Y4ÅHp|/ãÚóf6;ŒƒEaQaœ,ŒÎbÔ)ï°]06;‹FaQaœ,‹c|œú'ý'±±ØY0
‹Êâ"ÑXtããœ/9.ŒÅ£°¨,NEg1>N۔‹Åcgq°(0*‹FcÑYõ\ƒgc±Ã8X•ÅÉ¢Áè,Šó\ƒgc±Ã8X•ÅÉ¢Áè,‰gÞ¬]Ÿgc±Ã8XÆÉ¢Áè,‰~½dû‹Å£°¨0NE‡1HŒë%ûØXì,…EeqÂh,:ŒAa{Λý;`ƒ±³8`•Å	£±è,ŠíJP2l0v‹£²8a4Å@±_uê[l,v‹£²8Y4Å@q\uηØXì0…E…q²h0:‹A¢\uÚk6;ŒƒEaQaœ,ŒÎb¨×Ç重ÅÎâ€QXT'‹Æ¢Ã$ÎëãŒÃÆbgqÀ(,*‹FcÑaí³_‡
ÆÎâ€QXT'ŒÆ¢³(ú…f;l0v‹£²8a4Å@1.Ï%Ùáì0Feq²h0:‹a˜Ø^r|žÆÁ¢°¨0N
Fg1H<óf¶—"ϳÃ8XÆÉ¢±è0‰gÞÁöõì,…E…q²h,:ŒAâ™7C°%83ì,…EeqÂh,:ŒAâ™7#°½CË°³8`•Å	£±è,ŠgތÀ– ¿ÅÎâ`Q`T'ŒÆ¢³(žy3[ñ;ŒƒEQYœ,ŒÎb ø0ó•9®·Øa,
‹
ãdÑ`tƒÄ3o†`û8Ûkv‹Â¢Â8Y4Æ ñ̛!Ø>ÎþšÅ£°¨0NE‡1(Ïy3ÛÇ9;‹FaQYœ0‹cxæÍl0žkPà0
‹Êâ"ÑXtÅ3oF`ƒñ\ƒ
ç`Q`T'ŒÆ¢³(žy3‹ç'œŸç`Q`T'‹£³(ž3‹ç'´Ïs°(,*Œ"EƒÑYϼ'Åþ'þ…E…q²h,:ŒAâ™7C°±Øßa|€FaQaœ,‹cxæÍl0ö7(×8`•Å	£±è0‰gތÀcO°e8X•Å	£±è,ŠgތÀcO°g8X•Å	£±è,†ò0#°±Øoq°(0*‹"EƒÑYπÅž ¼ÅÁ¢°¨0N
Fg1H<óf6{úšƒEaQaœ,‹cxæÍl,ös¾æ€QXT'‹Æ¢Ã$žy3Œýã´×0
‹Êâ"ÑXtƒÄ3oF`ƒ±£é‡ƒEQYœ0‹Îb xæÍl0v4ãp°(0*‹"EƒÑYπÅã¾õ'S`T'‹£³(ž3‹Æs
68…E…q²h0:‹Aâ™7C°±Øa/Ù?OaQaœ,‹cP¨Ïy3‹ÅsIŽÏSXT'‹Æ¢Ã$žy3ŒÅñ'ò
‹Êâ"ÑXtƒÄ3oF`ƒ±³8^R?OQYœ0‹Îb xæÍl0vÇ;œ À¨,N
Fg1P<f6;ŒãÚ(0*‹"EƒÑYϼ'ÅãHÐ3ÆÉ¢Áè,‰gÞÁÆb‡q$
‹
ãdÑXtƒÄ3o†`c±³8¾Ÿóz‹Â¢Â8Y4Æ ñ̛Ø`ì,ŽÛ[•Å	£±è0‰gތÀcgqÔÙߢÀ¨,NEg10œÏy3ŒÅQçx‹£²8Y4Å@ñ˜ØXì0ŽS^S`T'‹£³$žy3‹Æñqêk
‹
ãdÑ`tƒÄ3o†`c±³8>Îy(,*Œ"EcÑaϼ'ÅÎâø8íPXT'‹Æ¢Ã$žy3ŒÅã¹NeqÂh,:ŒAâ™7#°ÁØYhÆ¡À¨,NEg1P<óf6;‹ƒÅ}IÚõy*‹"EƒÑYπÅã`ñ\'íóT'‹£³$žy3‹ÆÁ¢¼dÿ<ÆÉ¢Áè,…öœ7C°±ØY0ÊKŽÏSaœ,‹cxæÍl,vŒòåT'ŒÆ¢Ã$žy3ŒÅ£¼Cý•Å	£±è0‰gތÀcgq°(ïpf¨,NEg1P<óf6;‹ƒEy‡–¡²8Y4Å@ñ˜ØXì0åz†ÊâdÑ`tƒÄ3o†`c±Ã8X"#C…q²h0:‹Aâ™7C°±ØY0Ê÷Ó¯ÆÉ¢±è0‰gÞÁÆbgqÀ(u¶·¨,NE‡1H<óf6;‹F©³¿EeqÂh,:‹¡?çÍl0v‹'àx‹Êâ"ÑXtÅ3oF`ƒ±³8X":å5•ÅÉ¢Áè,ŠgÀŒÀÆb‡q°(uêk*‹"EƒÑYϼ'Åã`Q>Îùš
ãdÑ`tƒÄ3o†`c±³8`"Ó^Saœ,‹cxæÍl,vŒ'¦*‹FcÑaϼ
ÆÎâ€QЌCeqÂh,:‹â™7#°ÁØY,ʧס²8a4Å@ñ̛ØXì0Æs
68'‹£³(ž3‹ÆÁ¢Àx®ÁçdÑ`tƒÂxΛ!ØXì0Íq¨0N
Fg1H<óf6;‹Fañ\'òyNE‡1H<óf6;‹Fañ\'
ç"ÑXtƒÄ3oF`ƒ±³8`õ%çç9a4Å@ñ̛Ø`ì,F}Iû<'ŒÆ¢³(žy3‹ÆÁ¢À¨/éŸçdÑ`tÅ3`F`c±Ã8Xõ%ãœ,ŒÎbxæÍl,v‹Â¢þkÞ·6ëœ,ŒÎbxϛaØXì,…E}ÉöNE‡1HŒÆÆbgqÀ(,ê;ìà"ÑXtƒÁv]{àŒév'{€-dë{ŸòÛÈv²ëv'ÝÀîd²l}Ïò)O°l';°îٍìö [À֜5ëI¶ídÖã"»'ÝÁdÙúžg֓lÛÉ®å»'ÝÁdÙúž-ëI¶'í`×zÝÈîd°…lÍÙßõ$ÛÈv°ƒëyÝÈîd°…lÍ9²ž`ÙvpmÙ
ìNö[È֔ەõÛÈv²ë3Ès»"=È°õ3nïz'md;فõ™a乑ÝÁdØú÷w=É6°ì@º=çyndw°ÙB¶æ<Þõ$ÛÀv²ƒë3ÿˆs#»ƒ=Ȳ5gyדl#ÛÁ®Ïü#΍ìNö[ÈÖÏX¿åI¶'í`×gþ'çv'{€-dëg<ßõÛÈv°ƒë3ÿÈs»"=À²õ3¶w=Á6²ìÀúÌ?òÜÀîd²lÅØ¿å	¶'ídÖgþ'çFv{-`+Æñ-O²
l';°>óŽ<7²;؃l![?â~}˓lÛÉ®Ïü#΍ìö [ÈÖϸ}˓l#ÛÁ®Ïü#΍ìNö[ÈVŒŸóUgޑg#ÛÁ¦ûsþ'çv'{€-d+Æã[ž`Ùvp}æyn`w²Ù¶b,ßòÛÈv²ë3ÿÈs»"=È°•c}z'md;فõ™w乑ÝÁdØÊñ|z'm`;فõ™w乑ÝÁdي±==É6°ìàúÌ?âÜÈî`²…lÅ؟ždÙvp}æqndw²ØB¶bOO²l;¸>ó<7°;Ùl![)×Ól#ÛÁ®Ïü#Ï
ìNö [ÀVŽÛÓl#ÛɬÏü#Ï
ìNö [ÀVŽŸóTgþ'gÛɤÇsޑçFv{-`+ÇãéI¶ídÖgޑçFv{-d+Øçú–
l';¸>ó87²;؃l![Á>ׯ²ld;ØÁõ™őÝÉ`Ù
ö¹~'ËF¶ƒ\ŸùGž؝춐­ÛÓl#ÛÁ®Ïü#Ï
ìNö [ÀVŽýé	¶'ídÖgþ'çv'{-`+Ùçz–
l';°>óŽ<7²;؃l[ÉÞׯ\,ØNvp}æqndw°ÙB¶'}®ßƲíd×gþçFv{-d+Øçúí,Ùv0-ÏùGœٝ춐­`Ÿëw°ld;ØÁõ™乁ÝÉ`ÙJö¹že#ÛÁ®Ïü#Ï
ìNö [ÀV²Ïõ¬(ÙNv`}æyn`w²Ù¶'}®çɲídÖgޑçFv{-`+Ùçú5–
l';¸>ó87²;؃l![Á>ׯ³l`;ÙÁõ™őÝÉ`Ù
ö¹~ƒe#ÛÁ®Ïü#΍ìNö[ÈV°çK녲'í`×gþ'çv'{€-d+Ùçzn(Ùvp}æyn`w²Ù¶'}®çŽ²'ídÒúœ乁ÝÉdØJö¹žË¶"XŸyGžÙìA¶€­dŸëWX6°ìàúÌ?âÜÈî`²…lû\¿Ê²íd×gþçFv'{€-d+Øçú,Ùvp}æqndw²ØB¶'}®gCÙÈv°ƒë3ÿÈs»"=À²•ìs=;ÊF¶ƒ\ŸùGž؝ìA¶€­dŸë9P6²ìÀúÌ?òÜÀîd²l%{_ÏóbÙÀv²ë3ïÈs#»ƒ=È°•ìsý6–
l';¸>ó87²;؃l![Á>×ogÙÀv²ƒéùœőÝÉ`Ù
ö¹~ËF¶ƒ\ŸùGœٝ춐­ËÓl#ÛÁ®Ïü#Ï
ìNö[ÈVŽõé	¶'ídÖgþ'çv'{-`+Ùçzž(ÙNv`}æyn`w²Ù¶'}®gcÙÀv²ë3ïÈs#»ƒ=È°•ìsý:˶"\ŸùGœÙìA¶­`Ÿë7X6°ìàúÌ?âÜÈîd°…l{_¿v±ld;ØÁõ™őÝÉ`ÙÊq{z'md;ØÁõ™乁ÝÉ`ÙÊñs~êÌ?âld;ف´=çyn`w²Ù¶r<žž`ÙNv`}æyndw°Ù¶r,OO²
l';°>óŽ<7²;؃l[9Ö§'Ù¶"\ŸùGœÙìA¶­ϧ'Ù¶"\ŸùGœٝ춐­Ûӓl#ÛÁ®Ïü#΍ìNö[ÈVŒý[ž`Ùvp}æyn`w²ØB¶bßòÛÈv²ë3ÿÈs»"=È°b¿¾å	¶'ídÖgþ'çFv{-`+ÇíéI¶ídÖgޑçFv{-d+ÆÏù©3ÿȳídÓþœőÝÁdيñxz'm`;ÙÁõ™őÝÉ`ي±<=É6²ìàúÌ?âÜÈîd°…lÅX¿å	¶'í`×gþ'çv'{€-d+Æó[ž`ÙNv`}æyn`w²Ù¶blßòÛÈv²ë3ÿÈs#»ƒ=È°cÿ–'Ù¶"XŸyGžÙìA¶­Ÿq|˓lÛÉ®Ïü#΍ìö [È֏8®oy'md;ØÁõ™őÝÉ`Ùú·oy'md;ØÁõ™őÝÉ`Ùú÷w=Á6²ì`:žó<7°;Ùl![?ãñ®'ØF¶"XŸùGž؝ìA¶€­Ÿ±¼ë	¶'ídÖgþ'çFv{-`ëg¬ïz'm`;فõ™w乑ÝÁdٚó|דlÛÉ®Ïü#΍ìö [È֜í]O²l;¸>ó87²;Ùl![söw=É6²ìàúÌ?òÜÀîd°…l}Ïñ)O°l;¸>ó<7°;Ùl![ÿ}÷kÝÆþ'ØF¶"X¯ùGª؝ìA¶€­ï¹}Êl#Ûɬã"»'ÝÁdØúžû§<É6°ìºÝ1pÝÈî`²…l}íñ)O²
l';¸n؍ìö [ÈÖזOy'md;ØÁu¿Àndw²ØB¶¾¶~ʓl#ÛÁ®ÇEv»"=À²õµ'Êl#ÛÁ®å"»ÝÉdØúچòÛÈv²k½Èn`w²Ù¶¾¶£<Á6²ìÀz^d7²;؃l[_;PždØNv`mٍìö [ÈÞ×s»PždØNvp}æqndw°ÙBö¹žʓl#ÛÁ®Ïü#΍ìNö[È>×sGy'md;ØÁt{Î?òÜÀîd°…ìs=–'ØF¶ƒ\ŸùGž؝ìA¶`,O+Ùl#ÛɬÏü#Ï
ìNö [0Ö§•ìI¶ídÖgޑçFv{-ϧ•ìI¶ídÖgޑçFv{-Û·¬`O²
l';¸>ó87²;؃lÁØ¿e{'md;ØÁõ™őÝÉ`Æñ-+ؓl#ÛÁ®Ïü#Ï
ìNö[ î×·¬dO°l;¸>ó<7°;كlùŒÛ·¬dO°l';°>ó<7°;كlùŒû·¬dO²
l';îÏyGžÙìA¶ä<Þµ'=É6°ìàúÌ?âÜÈî`²%gÉZÁždØNvp}æqndw°ْ³f­`O²l;¸>ó87²;ÙlÉyf­`O²l;¸>ó<7°;ÙlÉÙ²V²'ØF¶ƒ\ŸùGž؝ìA¶¼gÏZɞ`ÙNv`}æyn`w²Ùòž#k%{'m`;فõ™w乑ÝÁdËKëSV²'Ù¶"\ŸùGœÙìA¶¼vCYÁždØNvp}æqndw²ØòÚe{'md;ØÁôxÎ?âÜÈîd°åµÊ
ö$ÛÈv°ƒë3ÿÈs»"=À–×"•ì	¶'í`×gþ'çv'{}®gEYɞ`ÙNv`}æyn`w²Çói[ɞdØNv`}æyndw°Çö´€­dO²
l';¸>ó87²;؃cZÈV°'Ù¶"\ŸùGœٝìq<-d+ؓl#ÛÁ®Ïü#΍ìNö€X®§…l%{'md;ØÁõ™乁ÝÉŸqû–…l%{'md;ØÁõ™乁ÝÉŸq׶'=Á6²ì@Zžó<7°;Ùã3ïZÀV²'Ù¶"XŸyGžÙìñË»°•ìI¶íd×gþçFv{|Æú®…l{'m`;ÙÁõ™őÝÉïyf-d+ؓl#ÛÁ®Ïü#΍ìNöxϖµ­dO°l;¸>ó<7°;Ùã={ÖB¶'=Á6²ìÀúÌ?òÜÀîd÷Ÿ²€­dO°l';°>ó<7°;Ùã¥õBYÀV²'Ù¶"XŸyGžÙìñÚ
e[ɞdØNvp}æqndw°Çkw"…l{'m`;ÙÁ´>çqndw²Ïõ<P²ìI¶'í`×gþçFvçXž`ÙJöÛÈv°ƒë3ÿÈs»s¬O°…l%{'md;فõ™乁Ý9žO²l%{'md;فõ™乑Ý1¶§Ù¶'=É6°ìÀúÌ;òÜÈ˃l[ɞdØNvp}æqnd÷Ï8¾åA¶­`O²
l';¸>ó87²ûG<¯w=À²ìI¶'í`×gþçFvϹe=À²•ì	¶'í`×gþ'çvϹg=À²•ì	¶'ídÒó9ÿÈs»ç<²dØJöÛÈv²ë3ÿÈs#»¿gÉz-`+ٓlÛɬϼ#ύìþÚú)²…l{'m`;ÙÁõ™őÝ_{~ʃl![ÁždØNvp}æqnd÷×6"ØB¶'=É6²ìàúÌ?âÜÈ>ׯ³<À²•ì	¶'í`×gþ'çö¹~ƒå¶­dO°l';°>ó<7°÷õk˃l[ɞ`ÙNv`}æyn·o¹ƒ=È°•ìI¶ídÖgޑç†qÿ–;؃l![ÁždØNv0mÏùGœÆã[î`²…l{'md;ØÁõ™Ĺ}Æò®;Ùl![ÁždÙvp}æqnŸ±¾ëNö[ÈV²'ØF¶ƒ\ŸùGž[Îó]w²ØB¶'=Á6²ìÀúÌ?òÜÞ³eÝÉdØJöÛÈv²ë3ÿÈs{Ïþ)w°Ù¶'=É6°ìÀúÌ;òÜÞs|ÊìA¶­`O²
l';¸>ó8·—öåö [ÈV°'ÙF¶ƒ\ŸùGœÛk7";Ùl![ÁždÙvp}æy>×sG¹"=À²•ì	¶'í`Óþœ"{<ÝÀîd°…l%{'md;فu»8–§؝ìA¶€­dO°l';°îÆú-7²;؃l[ɞdØNv`=.Œç·ÜÈî`²…l{'m`;ÙÁµ\Ÿ±}ˍìö [ÈV°'ÙF¶ƒ\땳¿ëFv'{€-d+ؓl#ÛÁ®ç•sdÝÀîd°…l%{'md;ØÁµ]o9®O¹ÝÉdØJöÛÈv²k¿Þsû"؝ìA¶€­dO°l';°Žë=÷O¹'ÝÁdØJö$ÛÀv²éxÎ;þ+"ÙìA¶­`O²
l';¸>ó!(7²;؃l![ÁždÙvp¬ÇgþçFv'{€-d+ؓl#ÛÁþåõò<>ó<7°;Ùl![ɞ`Ùö/¯_íøÌ?òÜÀîd²l%{'md;Ù¿¼ž"öoøÌ?òÜÀîd²l%{'m`;Ù¿¼ž"ŽoøÌ;òÜÈî`²l%{'m`;Ù¿¼žßq[·ßó=ïÈt#»ƒ=ȲìI¶ídÿòz~Ó-i¿Àndw°ÙB¶'=É6²ì_^¿ßpÿã»'ÝÉ`Ù
ö$ÛÈv°yý~Ãã~ü¢r]d7°;Ùl![ɞ`Ùö/¯ßc¹]d7°;كl[ɞ`ÙNö¹žä~'ÝÀîd²l%{'m`;Ùçzž ‹ìFv{-`+ٓlÛ9¶§ƒk¹Àndw°ÙB¶þïÞîž×¶]9ï|~?'nrԓ¬*²*mÃ:0`èf†ÒÜ×Ћa©¿¿'ùüi>ؽ{"‰ ZkŸQä«jŽyÙã±çeççq½u|.»=v¿l{lì¸ìñØó±ó׸þÈõÖãsÙí±ûcÛeûcÇeÇž¿ÄíóG®·fþñÛe÷ǶËöǎÇ—=;ÎíG]oÍüã;·Ëîmí—=.{>vþœûϺîšùÇwn—ÝÛÛ/;{<ö¼ìü1Û¯rÝt;óŽïÜ»_¶=¶_v<öxìyÙùcö_åzkæï¹=v¿l{lì¸ìñØó²ó÷·\oÍüã=·Çîm—폗={>6õ<n¹ÞšùÇ{nÝÛ.Û;.{<ö|ãyœ—]oÍüã;·Ëîm—폏=.{¾qçe×[3ÿøÎí²ûcÛcûeÇcËžw\ä|ìºkæß¹]vl{l¿ìxìñØó—¸þÈùØu×Ì;¾s{ì~ÙöØ~ÙñØã±çϹý¨ó±ë­™¼çöØý²í±ý±ã²ÇcÏsÿYçc×[3ÿxÏí±ûcÛeûcÇeÇž?fûUÎË®—îgþñžÛc÷ǶËöǎÇ—=ß~ËyÙõÖÌ?¾s»ìþØvÙþØñØã²çï;n9/»ÞšùÇwn—ÝÛÛ/;{\6õ;^9»îšùÇwn—ÝÛÛ/;{¼ñ<ž—]wͼã;·Çî—mí—=î8ÿÈó²ó±ë­™¼çöØý²í±ý±ã²Ç×y^v>v½5ó÷Ü»?¶]¶?v\öø%¶Ïz>v^v½5ó÷Ü»?¶]¶?v<öø9·õ|ì¼ìzkæß¹]vl»lìxìñcî?ëùØùØu×Ì?¾s»ìþØöØ~ÙñØã÷m¿Êó±ó±ë¦íÌ?¾s»ìþØöØ~ÙñØã÷í·</;»îšyÇwnÝ/ÛÛ/;›úWž—]oÍüã=·Çî—mí—MýŽWž—]oÍüã=·Çîm—íw<ÇcÏÇÎË®·fþñžÛc÷ǶËöǎ_ãüQËž—]oÍüã;·Ëîm—폿Æõ£—=;»îšùÇwn—ÝÛÛ/;~ÊþùYËž]wÍüã;·Çî—mí—?çö³=/;»îšyÇwnÝ/ÛÛ/;~ÌýWy<ö¼ì|ìzkæï¹=v¿l{llêÙny<ö¼ì|ìzi?ó÷Ü»?¶]¶?6õì·<{>v^v½5ó÷Ü»?¶]¶¿qÇcËž—]oÍüã;·Ëîm—íw<þÈñØã²çcçc×]3ÿøÎí²ûcÛcû¯ñü#ÇcËž]wÍüã;·Çî—mí?çüQÇcÇž—]wͼã;·Çî—mí?çúYÇeÇž—]oÍüã=·Çî—mí?äøü*ÇeÇž—]oÍüã=·Çîm—í¿ïvËqÙã±çcçe×[3ÿxÏí±ûcÛeûï»ßr<ö¸ìùØyÙõÖÌ?¾s»ìþØvÙÔ¯½r<ö¸ìùØùØuÓqæß¹]vl»cÿ#ûeÇcËž]wÍüã;·Çî—mwd¿ìxìñØó²ó±ë®™w|çöØý²í×xü¨ý±ã²ÇcÏËÎÇ®·fþñžÛc÷˶ŸóüYûcÇeÇž—]oÍüã=·Çîm?æüYûcÇeÇž—]oÍüã=·Çîm¿ïúUöǎÇ—=;/»ÞšùÇwn—Ý[õ<>·ì=.{>v>vÝ5óïÜ.»?6õÜ^Ù/;{\ö|ì|ìºkæß¹=v¿ã~lí—={^v>vÝ5óŽïÜ»ÿÛÙÛ;.{<ö¼ì|ìzéqæï¹=vÿ9ûÚÛ;.{<ö|ì¼ìzkæï¹=vÿ9ÇÏÚ.Û;.{<ö|ì¼ìzkæß¹]vÿ1_e»lìxìqÙó±ó²ë­™|çvÙý÷=oÙ.Û;{\ö|ì|ìºkæß¹]vÿ}ç-ÛcûeÇcËž]wÍüã;·7®ã~ÙöØ~ÙñØã±çeçc×]3ïøÎíŠççÜ/ÛÛ;.{<ö¼ì|ìzkæï¹ý·u¿l{lì¸ìñØó±ó²ë­™¼çökÜÔý±í²ý±ã²ÇcÏÇÎË®·fþñÛÙ~Öý±í²ý±ã±ÇeÏÇÎË®—žgþñÛïÛ•ûcÛcûeÇcËž]wÍüã;SÏqËý±í±ý²ã±ÇeÏÇÎÇ®»fÞñ©çñÊý²í±ý²ã±ÇcÏËÎÇ®»fÞñºçq{ì~ÙöØþØñÿÏÌÃÌÂô;óƒù{vvÌßRϟyî30õž3/—‰™ÈÂô·ªaþ~YúÿWçù´s?Pùï]3U‰wÿ»¯Çhy÷3úz•‹|ÿ>öÑóH_Yr'ØÈïy˜¾nûåÝïìëŸENå­ã"ß¿5ÝöuÛ&wò‰<q(ï¼û[}ý˜òþûe_ÇÖr×ói_Û¾ÜÈ6òÄN^x(·†§rë¸Èõû˜žGúºÌä}ÞôõÏ&;yâPî<•{ÃI®ßÇõ÷¾ÆúäF>ðÞ_:ߏk|tçû1ïí|ÿ•ñýoï¿1¾ß§ó~{ãû:ï·6ÞÇÝy¥ñ¾ÕÎûëŒ÷éuÞOc¼¿¨óytãýÏ£Ÿ?î|ÞÄø<YgÞÜø¼@gžÌ˜í̓ó>~'ÑÏíü½ØøûyçùÐø{Hç~иßíìÆ~ÖW[NvåÚ¾ʵ|=É
¹ÖO=wöƒ¯»®í_yáP®ýàë¡\ûÁ×Iî¸Èõÿ¯ô¼ÕÙ¾îä…÷<¨±|½ç}ŒýàëIn¸È÷úþÑß_ŒýàëNžØȇrí_ïùc?øz÷ïŒýàë"×úMû«±|ÝÉ»rí_‡rí_OrÃI®ß§ëïqÆ~à]û«±x×þjì_»ríÞµ¿ÚºläIî¸Èµ¾i5ö7Ý_Ûºä=nì_‡rïxNòÀE®õ]û«±|ݕëû1¿våÚœïC6¾ÿÆù¾Kc?p¾ÏÌx¿µó}5Æ~à|ñþ:çýÒÆ~à¼?ÔØœ÷ß?uÞÇcìÎûŒùrçó´Æ~à|>ʘ'qæߍýÀ™o4þ^ì̯ûÓŸ47õï<ï÷Îý›­ËVvåÚ¾äŽ'yà"×ï"Ú_ýà뮼>Øt½¨þ¿]OexNò‹\ë—öWc?øzﯾn3使:ûÁ×û¼õõŸYÞó+~ê¿´¿úº¬¿ŽöW§þ¿nÊÛ›rÕÿ×NnxžäïóÖ¹ˆ¦ýÕ©ÿ¯»òÞ°'rǃ|à$Ÿ¸Èõût·¾äýüàÜD×þêÔtí¯Îý@tí¯Ný]äú}Lû«SÿaÚ_û¯Üð>o}}¬@Þû«s?¦ýÕ©ÿ0í¯Îý@¸öW§þõ¿:÷áÚ_ú¾oÞ¹¾ßשÿàûú¾ŸË©ÿàûWœúÞ¯ïÜïKvê?x¦s?¼ïÌ©ÿà}6Îý@ðþ§þƒÏ‡:õ|ÞÇ©ÿ`žÛ©ÿ`^Ϲæ1œúúmÎý@ð÷S§þƒçW§þ¿v]Oªÿ¯ƒ|âIž8•«þ#µ¿:÷_7rÃFîØɺ^Tÿ_§®'Õÿ×{
ê?JûkPÿ_wrÇN8È'žä…÷yÔÿøèy&¨ÿ¯¹a#ìäòÄSy?ë—rÕÿhÚ_ƒúÿz?ÏõÿõÞ_ƒúÿ:È'ä…S¹õK¹êtí¯AýÝÉïó6¨ÿѵ¿õÿõT®ú]ûkpþÓþÔÿ׍<°'ìä‰÷yÔÿ0=Ïõÿu)×ù?\ûkPÿõ¿çÿ×F>qÊUÿƒïÇ
êð}"Áù?ø¾© þß'œÿƒ÷Åõ?xÿopþÞïÔÿàý]AýÞÏÜÿ>ÔÿàóŽÁù?øüJPÿƒùäàü̟õ?˜/êÐ?
îÿêÿk'/º^Tÿ_O]O:ÿ¿Nrý>©ý58ÿ¿näy⽿îÿ¿Þûë þ¿Þçíàþÿëý<3¨÷QÚ_çÿם<±'åºÿÿz(§þKûëàþÿë"ßëϏžg÷ÿ_ïýupÿÿµ+WýÊuÿÿõ$7œäû÷™Mûë Þ¿nä‰÷y;8ï¿ÞÏ3ƒúÿzNò³~'ë÷éÚ_õ>»ö×ÁýÿìÚ_çýìÚ_õ?»žgçýìÚ_õ>Mûëàþšö×A½OÓþ:¸ÿÿڕë¼ÿzžäK׋ê}ºžgÏÿ_wåª÷éÚ_隆®ýupÞ=È'ùÀE®õù~½Áy?ùþ¤A½O¾cPï"÷ŸÎûÉûlõ>y_á༟¼jPï"÷ÎûÉçÉõ>ùüÞ Þ'ŸÇœ÷"yÛA½Oæ©çý¤_>¨÷I?dPï_¹á <u½è¼ÿ:u½¨Þgjœ÷_ïýuRï_ïýuRï_;¹ãA>ð$Ÿ¸Èµ~鼝Ôû×{Ôû×Fî8Èò‰"ü¬_ÊUïùÑþ:©÷¯÷y;©÷¯÷ó̤޿ò‰'yâT®zϦýuRï_7rÃFîØÉÞÏ3"zÿzﯓzÿº"«Þ³kÔ{ví¯"zÏ®ýuRï_ùă¼ð>o'õž]Ï3"zOÓþ:9ßÓ´¿Nêýk'Ÿ8ÈOåª÷¯S¹Î÷tí¯"zO×ó̤ÞÓµ¿Nêýë O<"ë|O×þ:©÷äû­'õž|é¤Þ"率Ô{ò}@"ó=ù¾‡I½'ïóžœïÉûY'õž¼oRïÉû•&ç{òþŒI½'ŸžœïÉçÑ&õž|¾`RïÉüèä~>™šÔ{Òÿœï_y⽿&çû×{MîçsjMê=§ÎÛä|ÏÔþšÔûם<±+×ýüס\õþõ$7œäú}Jûkr¾½ÏÛä~þëý<"Ôû×®\÷ó_åÔ{iMîç¿.ò½~}´¿&õþu'/lÊUï_ïó6¹Ÿÿzï¯I}äûß«šö×ä~þëFžØ"ë~þkW®úþzÞçmr?_MÏ3I½W×þšÜÏݕ«¾¿6废¯®ý59Ï«kMêýë$?ë¹Ö7=Ï$÷ó_w]O:ÏË´¿&õ^¦ý5¹Ÿÿz'œäú÷rí¯ÉyþuS®zÿÚt½èïùåzžIê»\ûkr?ÿõ$?ë¹Öçûš"ó¼ø>Τ¾‹ï[Kþž_|ŸNržß_Ôwñ~êä</Þ7šÔwñ>¹äù½x_PržïƒHê»ø¼oržŸßJ께—OÎób²8ϋy—¢¾‹~gqžý΢¾‹~gQßE¿³8Ïkj-ê»èwçyÑï,ê»èwõ]ô;‹ó¼èwõ]ô;‹ó¼èwõ]¥ýµ¨ï¯<ð>oëÔ7ýÎ:õM¿³N}Óï,ÕwÿÐï,ç˝<°'Oä‰÷y[ªïåý<S:ϗ‹\ëÓï,Õ÷r'Øɇòøà©<Nr­O¿³TßË{-Õ÷²''vòÂCùhx*¹Ö7í¯¥ú^îº^ÆÄ®ëiå³á©|vœäZŸ~g©¾—ùÄF^ؕç]/ÙñÔõ"gý"×úô;Kõ½ÜÉ›òúàP^réë¥Îú¥ë©´>ýÎR}/¯ýuµá?xí¯öQ}/¹áI8ÉõßCóæˉ×óÌ×íƒ×þjÕ÷²"äŽ'ùY¿Èµþ¾QØ.ܕ÷†×y»lx=ÏØGõ½<ÈNò‰‹\ë«ßiݟ/wåÔwíýuÙñ:o—^Ï3k‹|¯ßÔïüZõÝÔﴏÎïe#wäùÄI~Ö_ç­}¨ï¦~§}t¾ÜÉ
;yà Ÿx''NåCë÷½¿.wÜt½æëevò‰yâ©|žõK¹ê»©ß¹l¸"6òC×ËL<t=©ž›úöÑýùr'k}õ;íC=7õ;—vòÄA^xêz©†Sד깩ßiݟ/7ò<±"^û«5ê¹éûN–ÏúE®õÕï´F=7õ;—'vò¡\õÜÔï\î8ɵ¾úË7ò‰×ykznêw®1†‡òÞñ$?ë¹þ{¨ß¹<q'/lÊíƒC¹ê¹©ß¹ìxí¯Ö8¯›úÖ¨ç¦~§µSÏêw®±¢våÔsimœ×­´¿¶SÏêwZ£ž»úË‰›rÕsW¿ÓõÜÕï\6<ÈOò³~'k}õ;­QÏ]ýÎ厍Üpä'ùY¿"«ž5¨µÝp'7ìº^TÏüÙx''.åªg
–l7ÜÉ
yà xèzQ=«1¿\gýR®zîêwZ£žÕøÝvìäyâI^xﯝzVãlÛðÞ_;õ¬FÑöÀNžxžÊÛY¿"ë|îz»1O×õ‡îí×óŒ1?×õ‡]Æàä¡\õÜÕï4æç:Ÿ/\Öúêwósy`c~nÙɯçc~®ë3Û'¹ÖW¿Ó:ç³þ°=±'våºßփçvÇû¼íœÏzÐÚÖúêwZ?õ¬~§1/×uc¿¬ûí®~§õSÏêwór]7'Û{}ÝÈmOÜt½è~[7.{Ì°aW®z6õ;5†(Oò³~'k}õ;ù¸®z-6lº^t¿­iÛñ 8ÉÏúE®õÕï´NýšúÆ|\׈mÇ¡ëEõlêw.OœäZ_ýNëÔ³©ßiÌÃ-¹c'<È'žägý}Þ2×MýNcn¹";6òÀA>ñ /œÊÛY¿"ë<6õ;ù·åõ<³ØÉ'䅧òþÁ¥\籩߹츓6ò‰÷y˼ÛòÞ_óØÔï\>ë¹ÖW¿ÓŒóØÔï4æݖ¼p(×ylêwónËûyƨ_S¿Ó˜w[näyaW®óØÔï\îx'Ÿõ‹\ë«ßivêWýN³S¿êwómË¡œúU¿ÓìÔ¯úÆ|Ûr'ïõý£ýÕ¨_W¿Ó˜o[v]Oª_W¿Ó˜g[žä"\ë«ßi̳-7å:½iežmÙÉ]/ª_W¿Ó˜g[.r­¯~ç*³†»rÕ¯«ß©2"ƒ|àI>qêzQýºúÆüÚòÞ_™_[6rÇN>ð Ÿx'ŸõK¹Î_wí¯Ì¯-ïç§~]ýNc^m9È'ä…Sy?ë—rÕ¯‡öWæՖ;ùÀû¼e^myï¯Ì«-Oå:]ýNc^­»úÆ¼Úr#ØÈ'vòÂû¼e>my?Ï0Ÿ¶\äZ_ýNc>m¹"'6ò¡\çT®ûgŸÚ_™Oë®~§9篫ßiÎý³«ßi̧-»r¿®~§1¶<ÉÏúE®õKû+óhË]×õ«~§1¶Êuÿìêw.Nò³~'ïõCýNcþl¹+×ù»æ)É
‡®Õk¨ßiÎýs¨ßi̟õP¿Ó˜?[nÊU¿¡~§1¶ìäùÀS×Kõ÷óLpކúÆüÙr'7l䁃|âAž8•·³~)W½†úÆ¼ÙòÞ_™7[vò‰ƒ<ñT®ó6Ôï\Öúêwófˍ<ð>o™/[ÞÏ3̗-å:oCýNc¾l¹È÷õêwóe˝|b'/ÊuކúÆ|ÙòÞ_ƒz
õ;ù²åF>±'våª×Ðû=—;žägý}Þ2OÖCýNcžl¹"6åª×P¿Ó˜'[䎓ü¬_äúï©~§õêwócË®\õêwZpކúÆüØr'k}õ;ù±å¦œz-í¯qêUýN‹S¯êwZœzU¿ÓâÔ«úÆ¼XêwZP¯CýNc^lÙÈùÀS׋êu¨ßi̋õ¡~§
Îס~§1/¶l䁝|âAžx*ogýR®zêwÚ ^‡ú6¨×¡~§1¶䅇rÕëP¿Ó˜[.òýßs˜öWæÖ÷yË|Øò~žÔëP¿Ó˜[žÊU¯CýNÔëP¿Ó˜[näyaW®óu¨ßĩ-ïý•y°å"×úêwÚà|êwó`˦\õ:Ôï4濖¹ã}Þêu¨ßiÌõ¡~§1ÿµÜ•«^‡úÆü×ržä'¹Ö×ûflp?<ÔïÔǾdÓõ¤zêwÚà|êwó^ËI~Ö/å:_GjeÞk¹";v]/ª×¡~§1ïµ<ɧrêUýNcÞk¹';6ò|â¡ëE÷ÃCýNc¾kyﯓzêwó]˝|`#O䅇rݯyJåªÏ©~§1ßÕ§ú6¹žêwêcw²+W}Nõ;mr?<Õï4湖"|ÿ{Ï®ýur?<Õï4湖÷óó\Ë®\õ9Õï4湖'ùY¿È÷¿÷T¿Ó˜ßZîÊužNÓþÊüÖò>o™ßZÞûëä<êwó[}ªßiÌo-7åªÏ©~§1¿µìäŽùÀû¼e~ky?ÏLÎÓ©~§MêsªßiÌk-¹ã x'NåªÏ©ï¯5æµúT¿Ó˜×ZTŸ"~'óZËAžx*W}NúÌgõI¿sržN½?Å&õ9éw2ŸµìºžTŸ"~'óYËSyõ‹\ÿô;™ÏZîäy὿&õ9éwæ©Oúyê"~gžú¤ß™§>éwæ©Oúyê³´¿æ©ÏÒþšœŸ"~'óX=éw2µÜ•«>"~'óXËAnxNò‰‹\ëÓïdþjy?Ï0µì䎃<ð$Ÿ8É÷¿GÒïLÎÏìÚ_™¿Z6rÇû¼eÞjyï¯I}&ýΤ>"~'óV=éw2oµÜÉùÀAžxŸ·Éù™ô;™·Z.r­O¿39?"~'óUËNž8"«>Óµ¿2_µœäúyéw2_µÜt=éüLúÌW-»rÝß&ýN櫖'ùY¿Èõï¡ïc5橖»®ÕgÒïdžj9"ëþ6éw&õ™ô;™§êI¿"yªå½¿÷·©÷óTËNnx?Ï÷·I¿³¸¿MúÌSõ¤ßYÜß&ýN槖Üqäïó–ù©åý<S§éw2?µÜÉ;ùÀAžx'N庿]ó"Êu^ýÎ3/Uô;‹ûÛ¢ßy楊~癗*úE=ýÎ3/µæ+Éwò‰÷y[ÔcÑï<óRE¿³8/‹~癏*úg>ªèwçeÑï<óQÕµ¿žù¨¢ßYÔcÑï<óQE¿óÌGý΢‹~gQE¿óÌGýÎâ¼,Óþzæ¡Ê´¿žy¨¢ßYœ—E¿óÌCýÎ3Uô;Ï<TÑï,ê±èwžy¨¢ßYÔc…ö×¢‹~ç™*úE=ý΢‹~ç™*õ;ýÌ?•ú~æŸJýN?óO¥ïõ3ÿTúþ8ÿP¥~§Ÿù§R¿ÓÏüS©ß¹Üq'ëçU¿s9p'ŸØɇrÕc©ßéê±Ôïô3ïTêwú™w*õ;—›r¥~§Ÿy§R¿Ó?§÷FÌkä"×Ï«~çr⵿ú™o*õ;ýÌ7•ú~æ›JýN?óM¥~§3ßdõ;ù¦å¦|ŸËë¼u曖×óŒTËƒ|àIž¸"ïóÑ>êwúGõ¸ÜÉ
yà Ÿxèz‰S×Ó<ë—ò©ŸWýNµYäNØÉ'òÂSy6œº^R?¯úËŽùÀFžØ•×åÕð$?ë¹~^õ;—'îº^ªðÚ_½©—×þêM÷«ËƒÜq'\äZ?öþêÌ+-wå­áuÞzÓýêòÚ_y¥åI>p'ëßCýÎõšîÊ{ÇFn8ȯó֙OZ^Ï3Î|Òr)7­¯~§3Ÿ´ÜÉ;ùÀAžx'Nå®õ;y¤åµ¿:óHËF>±"'ÊョrêOýNo§þJû+óHËë¼u摖×óÌráPNý©ßéíԟúËgý"ßÿMýNgþh¹+Wý}íÊ÷y¸º^öy¸<u=©þšúÎû½¬©ßé¼ßk¹)Ï6åû<\vrǃ|àÔõ¢úkêw:ïó²¦~§3o´Ü•«þšúÎû»–ƒ|àIžxﯼ¿Ëšiåý]Ëëyƙ/ZÞû+ïïZvò‰yá©\õ×Ôït括©ßéÌ-wò÷yË|ÑòzžqÞϵ<"«þšúÎ|Ñr'ëçU¿Ó;õ×Ôït扖]¹ê¯©ßéÌ-¯çgžh9Éõóªßé¼k¹'6媿¦~§óþ­åAx'O¼Ï[Þ¿eMýÎÕÖþà®\õ×Ôït懖ƒ|àA>q'.媿¦~§ó~­eÓõ¢ó¯©ßéýԟúÞOý©ß©¶»\Êuþ5õ;y¡åNØÈ']/ԟúÎ¼Ðr*×ù×Ôït慬«ßé¼?k¹"'vå:ÿúGû+óAËS׋꯫ßéÌYW¿Ó™Znäëçýë?­ƒïóÛ?o¿}öÿþ×ÿúßíÿ»½ïîñƒØÞû.sC˃Üñ$¸Èõ{¨êÌ	™^`·Ý°'òÀƒ|â$/\Ê»Ö3í»Ì	™^pµíx=ç8ïÅ2½Ði;ñT®:ìêƒ:ïÅ2½0hÛp#lä;yáõœãÌ™^¸²Ýq'ëçUTãr'Oìä…C¹îKõ	^·%ïs˜9 Ó¶'nä…M¹îKõü펹ãI>p'ëçÕ{è9 Óœ—uvõA÷Z™>лxOœägýR®spÍY*×9¨Ln;v]/Ô¡ú n§Õuæ~LˆkÎ܏éiۆy`#ŸØÉïsØ9õŸíŽ‹|ÿ¼¦>¨3çcú€Évb#/ÊUokîR¹êÍ>Úwy/•™ú Î\ÏòÞwy/•i€}¿níƒ]¹êMÜێ'ùÀE®õºö]æzL»Ëª7
ÌnòÀƒ|â$?ë•r՛©ºÜq'wìäïçæxLjûurg½T®zӀֶáFØÈ'vòÂC¹êM2ÛïçævL"ÛwòĦ\瞩êÌ혶
'yà"×Ï«>¨óÞ(SÃx¿>¯aW®z3õA÷F-Oò"\?¯ú ÎœÎrS®sO
¬máëIõfêƒjÜLNòÂ{e.ÇL}Pg.Çô~^ÿ';ùÀAžx?ç0—cúƒosærLpÝvÜÈùÄN^x(×ù¶þ¦\÷™¦>¨3‡cúÑöÀ<±)×ù¦?Xlw<È'ùY¯Èµžú ÎÎò~Î	î3õ€×œ÷:-yàI>q'k=õA×øß7åºÏ\7¸äŽ÷yËÜÍòÞ_ƒ¿³è†m¿žñ¬WÊuŸéêƒ.î䁍|â /<u½Ì³^êzQ}i£ßvÜÈ6òÄ®\ç™6†íŽ'ùY¯Èõóª꼗Ét!m6å:Ï\}Pg®fyŸõ'ü¬Wäúy‡öWæj–÷yË\Íò~Îԗ«ê¼wiy'Ÿõ'\?¯ú Î{—–›rg®÷";s4ËN>ñ~ÎaŽfy﯃úrõA9sõA9šåN>°''åÔWj§¾ÔõqêK}Pç½Jæêƒ:s3˝¼°+§¾Ô]6<ÉÏzI¾×[ï±$O¼ŸsxoÒòÞ_yoÒr;ä'ùY¯"«¾Öœ¥rÕW4í¯ÌÉ,»®ÕW¨êƒú
õA÷"-§rÕW¨êÌÅ,7rÇF>°"'º^T_¡>¨3³\äZO}Pœ_¡>¨óÞ£e#/ÊU_aÚ_yïÑr'.]/ª¯PԙƒYÞû+s0Ë{ef9ÈOò"\?ohœ_¡>¨ó^£åý<ÃÜ˲"äOòÂ¥\õêƒ:s/˝<°'O¼ÏÛÉýa¨ê̽,§rÕW¨ê¼·h¹'lä‰]¹îcjeÎeyŸ·Ì¹,ïçæ\,ÔõyêK}PgÎeٔëþ0Ô]6<ÈÏzI~Ö+r­§>¨ÏS_êƒ:ï%ZvrÇA>ð$OœÊu8ÔõÉßEÆGû+ïZ6]/º?êƒ.O<ÈOåº?êƒ:s,6ÔuæX–;ùÄF^8"ëþp¨ê̱,§®§r\äû÷êƒ:ïZÞû+ïZÞû+s+ËAîx'ÞçmòwÈ¡>¨3·²Ü•ë¼êƒ:s+ËAxŸõ'ü¬WÊUOC}Pç½AËûy†÷-;ùÀAžx*W=
õA9êƒ:s*ˍ|`#O¼Ï[æT–÷þʜÊòT®ójÐå½@6èƒ2—²ÜÉ›rÕÓÚ_™KYÞçmROƒ>(s)ËE®Ÿ—>(s)Ë]¹êiÐå½?ËA>ð$?ë¥rê‰>hžz¢šœWƒ>hžz¢š§žèƒæ©'ú yê‰>hžz*í¯yê‰>hžz¢š§žèƒæ©'ú yê‰>(s'6éƒ2w²ÜÈïý•¹"彿õ4éƒòޞ彿òޞå"×zôAyoÏrW®zšôA‹zšôA™3Yäïó–9"åý<܉Mú Åù4éƒò^že'Ÿ8ÈO媧ٵ¿ò^›¦ýµ¨§I"¹'彿2W²ìÊu>Mú Ì•,Oò³^'k=×þÊ\Ér'/¼Ï[Þ»³¼ŸgxïÎò œäg½"×zôA™#YîÊu¿7Cûkq¿7éƒò^å©ëEõ4éƒ2Gb">(ïÕYî䎍|à O<"çY/•çY¯t½è~oÒend¹"'vò¡\÷{">(s#ËI®ß?µ¿òޜå¦ëE÷{S}Ð`Ndyí¯ÁœÈò ?ëMò³^'k=õAãsêgTmwläŽ×y¼gyí¯Á{q–S¹þ8Õ
æB,Õ
æB–;ùÀNž8"«~R}Ðà½7Ëëy&xú Á\Èr#ŸØÈ»rG©>h|8r7T·ÏzE®õԍ3'êƒÆ™IõAƒ÷Ú,yàI~ÖKrýþêƒÆ™ÉÝÙîx·ËŽ×óL|8R}Ð8s©>hœ¹T4ÎÜGªgî#Õ
Þ[³lä‰C¹ê'Սõ"êƒÆ™óHõAƒ÷ÖXªªçɝ¼°+WýäþÀÔ¶áI~ÖK]/ªŸT4ΜGª¼—fyí¯Á{i–<ð ?ëMò³^)Wý¤ú Á{h–×óLœ¹ŽT4Î\Gªg®#Ս3בêƒÆ™ëHõA£úÙ/œÜ¸"'^çmœ9ŽT4ÎGªgŽ#Ս3ǑêƒÆ™ãHõAƒ÷Ê,›rêg$n^çmœ9ŽT4ÎGªú)õA£Q?¥>hð™e'äOò³^*×ùSêƒÆ™Û(õAƒ÷Æ,ùÄN^x(Ÿg½©\õSêwF£~ªkå=1Ë]׋ê§ÔïŒ3§QêwƙÓ(õ;ãÌi"úqæ4JýÎ8s¥~gð^˜å®\÷oeÚ_yÌrèzÑý[©ßg.£ÔïŒ3—QêwƙË(õ;ãÌe"úqæ2JýÎ8såÚ_Ï\F©ßg.£ÔïŒ3—Qêwߛ¶ÜÉ'vò¡\÷o¥~gœ9Œ
í¯g£†ö×3‡QêwƙÃ(õ;ƒ÷º,»rõŸJýÎà{Ж'ùY¯Èµžúqæ.Jߣgî¢ÔïÞã²¼žg'÷¸,òÄ©\¯+õ;ãÌ]"úqæ.JýÎ8s•Ú_ù^³å}Þò½fËëy&xOËr'k=õ;ãÌY"úqæ,JýÎ8s¥~gœ9‹*í¯g΢Jûk?õ¢~gð=eþQ¿3øž²å®|×˲';òùY/É—ò}ÞøGýÎ`®bÙt½ìófÙÉ'ä…÷þj:o–÷þÊ÷ŽùGýÎà=+˝|b#/¼Ï[æ%–÷þ'Är'ŸõŠ\ë©ßÌK,wå½aWÞ
yà}Þò•åõ<¼GÅ?êwóËM¹6òµÞ_ÿéÿúóŸ>Œžü¯ÿùÏÿùÿôþÛïÿÝoþ»ßÚÞ{>ÿóÈ{bÌ~3}ãǟÿá·¿úþéïÿæŸþßùíŸÿÓ?ü·¿ÿÛþW¿ýù¿þéßüyý?øÁ¥ÚþÛÓZêÿøíþéoþöïûoÿýoÿæ/ÿù_þòOÿøã«å¾û_?×ø«ùïÿê·ï&öWÿé/ÿø—ü/ÿóçû¿ýùÿþÿ´äÿþóýÝ_þåü`ÿþOÿ¦ðÞendstream
endobj
3 0 obj
<< /Type /Pages /Kids [ 7 0 R ] /Count 1 /MediaBox [0 0 432 360] >>
endobj
4 0 obj
<<
/ProcSet [/PDF /Text]
/Font << /F1 10 0 R /F2 11 0 R >>
/ExtGState << >>
/ColorSpace << /sRGB 5 0 R >>
>>
endobj
5 0 obj
[/ICCBased 6 0 R]
endobj
6 0 obj
<< /Alternate /DeviceRGB /N 3 /Length 2596 /Filter /FlateDecode >>
stream
xœ–wTSهϽ7½P'Š"ÐkhRH
½H'.*1	JÀ"6DTpDQ'¦2(à€£C'±"Š…Q±ëDÔqp–Id­ß¼yï͛ß÷~kŸ½ÏÝgï}ÖºüƒÂLX	€¡Xáçň‹g`ðlàp³³BøF™|،l™ø½º ùû*Ó?ŒÁÿŸ"¹Y"1P˜ŒçòøÙ\É8=Wœ%·Oɘ¶4MÎ0JÎ"Y'2V"sò,[|ö™e9ó2"<ËsÎâeðäÜ'ã9¾Œ'`çø¹2¾&cƒtI†@Æoä±|N6('Ü.æsSdl-c'(2'-ãyàHÉ_ðÒ/XÌÏËÅÎÌZ.$§ˆ&\S†"‹áÏÏMç‹ÅÌ07#â1ؙYárfÏüYym²";Ø8980m-m¾(Ô]ü›'÷v–^"îDøÃöW~™
°¦eµÙú‡mi]ëP»ý‡Í`/Š²¾u}qº|^RÄâ,g+«ÜÜ\KŸk)/èïúŸC_|ÏR¾Ýïåaxó"8't1C^7nfz¦DÄÈÎâpù柇øþuü$¾ˆ/"ED˦L L–µ[Ȉ™B†@øŸšøÃþ¤Ù¹–‰ÚøЖX¥!@~(* 	{d+Ðï}ÆGù͋љ˜ûςþ}W¸LþÈ$ŽcGD2¸QÎìšüZ4 E@ê@èÀ¶À¸àA(ˆq`1à'D €µ "'­`'¨u 4ƒ6ptcà48.Ë`ÜR0ž€)ð
Ì@"…ÈR‡t CȲ…XäCP"%CBH@ë R¨ª†ê¡fè[è(tº
C· Qhúz#0	¦ÁZ°l³`O8Ž"ÁÉð28.'·À•p|î"O×àX
?§€:¢‹0ÂFB'x$	!«¤i@ڐ¤¹ŠH'§È[EE1PL"Ê…⢖¡V¡6£ªQP¨>ÔUÔ(j
õMFk¢ÍÑÎèt,:‹.FW ›Ðè³èô8úƒ¡cŒ1ŽL&³³³ӎ9…ƌa¦±X¬:ÖëŠ
År°bl1¶
{{{;Ž}ƒ#âtp¶8_\<Nˆ+ÄUàZp'pWp¸¼ÞïŒÅóðËñeøF|~?ŽŸ!(Œ	®"HB*a-¡'ÐF8K¸KxA$õˆNÄp¢€¸†XI<D<O%¾%QHf$6)$!m!í'"Ý"½ "ÉFdr<YLÞBn&Ÿ!ß'¿Q *X*(ðV+Ô(t*\Qx¦ˆW4TôT\¬˜¯X¡xDqHñ©^ÉH‰­ÄQZ¥T£tTé†Ò´2UÙF9T9Cy³r‹òåG,ňâCáQŠ(û(g(cT"ªOeS¹ÔuÔFêYê8
C3¦ÐRi¥´ohƒ´)ŠŠJ´JžJÊq)¡Ñèéô2úaúuú;U-UOU¾ê&Õ6Õ+ª¯Õæ¨y¨ñÕJÔÚÕFÔÞ©3Ô}ÔÓÔ·©w©ßÓ@i˜i"käjìÑ8«ñtmŽË9‡çÜք5Í4#4WhîÓМÖÒÖòÓÊÒªÒ:£õT›®í¡ª½Cû"ö¤UÇMG ³Cç¤Îc†
ӑΨdô1¦t5uýu%ºõºƒº3zÆzQz…zíz÷ô	ú,ý$ýú½úS:!­·
ñ†,ÃÃ]†ý†¯ŒbŒ6u=2V30Î7n5¾kB6q7YfÒ`rÍcÊ2M3ÝmzÙ6³7K1«12‡ÍÌæ»Í‡-ÐNB‹‹Lӓ™ÃleŽZÒ-ƒ--»,ŸYXÅ[m³ê·úhmonÝh}džbhShÓc󫭙-׶ÆöÚ\ò\ß¹«çvÏ}ngnÇ·ÛcwӞjb¿Á¾×þƒƒ£ƒÈ¡ÍaÒÑÀ1ѱÖñ‹Æ
cmfwB;y9­v:æôÖÙÁYì|Øù¦KšK‹Ë£yÆóøó獹ê¹r\ë]¥n·D·½nRw]wŽ{ƒû}žG"Ç"§©gªçAÏg^Ö^"¯¯×lgöJö)oÄÛÏ»Ä{ЇâåSísßWÏ7Ù·ÕwÊÏÞo…ß)´ÿ6ÿZ܀怩@ÇÀ•}A¤ AÕA'Í'EÁ=!pH`Èö»ó
ççw…'ЀÐí¡÷΅…}Ž	¯	aQÑ¿€º`ɂ–¯"½"Ë"ïD™DI¢z££¢›£_ÇxǔÇHc­bWÆ^ŠÓˆÄuÇcã£ã›â§ú,ܹp<Á>¡8áú"ãEy‹.,ÖXœ¾øøÅ%œ%Gщ1‰-‰ï9¡œÎôҀ¥µK§¸lî.îžoo'ïÊ/çO$¹&•'=JvMޞ<™âžR'òTÀTž§ú§Ö¥¾NM۟ö)=&½=—'˜qTH¦	û2µ3ó2‡³Ì³Š³¤Ëœ—í\6%
5eCً²»Å4ÙÏԀÄD²^2šã–S"ó&7:÷Hžrž0o`¹ÙòMË'ò}ó¿^ZÁ]Ñ[ [°¶`t¥çÊúUЪ¥«zWë¯.Z=¾Æóµ"µik(´.,/|¹.f]O'Vњ¢±õ~ë[‹ŠEÅ76¸l¨ÛˆÚ(Ø8¸iMKx%K­K+Jßoæn¾ø•ÍW•_}ڒ´e°Ì¡lÏVÌVáÖëÛÜ·(W.Ï/Û²½scGɎ—;—ì¼PaWQ·‹°K²KZ\Ù]ePµµê}uJõHWM{­fí¦Ú×»y»¯ìñØÓV§UWZ÷n¯`ïÍz¿úΣ†Š}˜}9û6F7öÍúº¹I£©´éÃ~á~遈}͎ÍÍ-š-e­p«¤uò`ÂÁËßxÓÝÆl«o§·—‡$‡›øíõÃA‡{°Ž´}gø]mµ£¤ê\Þ9ՕÒ%íŽë>x´·Ç¥§ã{Ëï÷Ó=Vs\åxÙ	‰¢ŸN柜>•uêééäÓc½Kz=s­/¼oðlÐÙóç|ϝé÷ì?yÞõü±ÎŽ^d]ìºäp©sÀ~ ãû:;‡‡º/;]îž7|âŠû•ÓW½¯ž»píÒÈü'áëQ×oÞH¸!½É»ùèVú­ç·snÏÜYs}·äžÒ½Šûš÷~4ý±]ê =>ê=:ð`Áƒ;cܱ'?eÿô~¼è!ùańÎDó#ÛGÇ&}'/?^øxüI֓™§Å?+ÿ\ûÌäÙw¿xü20;5þ\ôüÓ¯›_¨¿ØÿÒîeïtØôýW¯f^—¼Qsà-ëmÿ»˜w3¹ï±ï+?˜~èùôñOŸ~÷"óûendstream
endobj
9 0 obj
<<
/Type /Encoding /BaseEncoding /WinAnsiEncoding
/Differences [ 45/minus 96/quoteleft
144/dotlessi /grave /acute /circumflex /tilde /macron /breve /dotaccent
/dieresis /.notdef /ring /cedilla /.notdef /hungarumlaut /ogonek /caron /space]
>>
endobj
10 0 obj
<< /Type /Font /Subtype /Type1 /Name /F1 /BaseFont /ZapfDingbats >>
endobj
11 0 obj
<< /Type /Font /Subtype /Type1 /Name /F2 /BaseFont /Helvetica
/Encoding 9 0 R >>
endobj
xref
0 12
0000000000 65535 f 
0000000021 00000 n 
0000000164 00000 n 
0000031684 00000 n 
0000031767 00000 n 
0000031891 00000 n 
0000031924 00000 n 
0000000213 00000 n 
0000000293 00000 n 
0000034619 00000 n 
0000034876 00000 n 
0000034960 00000 n 
trailer
<< /Size 12 /Info 1 0 R /Root 2 0 R >>
startxref
35057
%%EOF

